Parameter-Efficient Transfer Learning for NLP

Fine-tuning large pre-trained models is an effective transfer mechanism in NLP. However, in the presence of many downstream tasks, fine-tuning is parameter inefficient: an entire new model is required for every task. As an alternative, we propose transfer with adapter modules. Adapter modules yield a compact and extensible model; they add only a few trainable parameters per task, and new tasks can be added without revisiting previous ones. The parameters of the original network remain fixed, yielding a high degree of parameter sharing. To demonstrate adapter's effectiveness, we transfer the recently proposed BERT Transformer model to 26 diverse text classification tasks, including the GLUE benchmark. Adapters attain near state-of-the-art performance, whilst adding only a few parameters per task. On GLUE, we attain within 0.4% of the performance of full fine-tuning, adding only 3.6% parameters per task. By contrast, fine-tuning trains 100% of the parameters per task.

==> content/conclusions.tex <==
\section{Conclusion}

We propose a transfer strategy for large text models using bottleneck adapter modules.
Adapter tuning yields models that are competitive with state-of-the-art fine-tuning, whilst using only small number of task-specific parameters.
This strategy is designed for an online setting, where tasks arrive in series, and one wants to solve them with a single model.
For future work, adapters could be applied in multi-task training, where tasks are available simultaneously.
Adapter modules could learn task-specific features while the main network learns generalizable representations.
Unlike traditional approaches that use a task specific network ``head'',
adapters allow task-dependent modulation at any layer.

